Optimal Advertising for Information Products

When selling information products, the seller can provide some free partial information to change people's valuations so that the overall revenue can possibly be increased. We study the general problem of advertising information products by revealing partial information. We consider buyers who are decision-makers. The outcomes of the decision problems depend on the state of the world that is unknown to the buyers. The buyers can make their own observations and thus can hold different personal beliefs about the state of the world. There is an information seller who has access to the state of the world. The seller can promote the information by revealing some partial information. We assume that the seller chooses a long-term advertising strategy and then commits to it. The seller's goal is to maximize the expected revenue. We study the problem in two settings. (1) The seller targets buyers of a certain type. In this case, finding the optimal advertising strategy is equivalent to finding the concave closure of a simple function. The function is a product of two quantities, the likelihood ratio and the cost of uncertainty. Based on this observation, we prove some properties of the optimal mechanism, which allow us to solve for the optimal mechanism by a finite-size convex program. The convex program will have a polynomial-size if the state of the world has a constant number of possible realizations or the buyers face a decision problem with a constant number of options. For the general problem, we prove that it is NP-hard to find the optimal mechanism. (2) When the seller faces buyers of different types and only knows the distribution of their types, we provide an approximation algorithm when it is not too hard to predict the possible type of buyers who will make the purchase. For the general problem, we prove that it is NP-hard to find a constant-factor approximation.

==> related.tex <==
\begin{comment}
	

\section{Optimal Information Disclosure}

There is a sender endowed with a prospect, which is randomly drawn from a finite set $P=\{1, \dots, N\}$. The probability of $i$ being realized is $p_i > 0$ and $\sum_{i=1}^n p_i = 1$. Each $i\in P$ is characterized by its payoffs $(\pi_i, v_i) \in \mathbb{R}^2$, where $\pi_i$ is the prospect's profitability for the sender, and $v_i$ is  its value to the receiver.

The sender chooses a disclosure rule $\langle \sigma, S \rangle$ to send a signal $s\in S$ drawn from $\sigma(i)$. The receiver observes the signal $s$, and decides whether to ``accept'' ($a=1$) or `` not accept'' ($a=0$). The receiver forgoes an outside option worth $r\in \mathbb{R}$, which is a random variable independent of $i$. So the sender's payoff is $a \cdot \pi$ and the receiver's payoff is $a(v-r)$.

Assume $v\in[0,1]$ and $r \sim \mathcal{U}[0,1]$. Then the sender's expected payoff is 
\begin{align} \label{optimal_info_dis}
\E_{s} \big( \E[\pi|s] \cdot \E[v|s]\big) = \sum_s \left(\sum_i p_i \sigma(i, s) \right) \frac{\sum_i p_i \sigma(i, s) \pi_i}{\sum_i p_i \sigma(i, s)} \cdot \frac{\sum_i p_i \sigma(i, s)v_i}{\sum_i p_i \sigma(i, s)}.
\end{align}

\paragraph{Optimal Information Disclosure as \sherry{Optimal Advertising?}.} Consider a Optimal Advertising problem with a common buyer prior belief. Let the state of the world be the realization of the prospect, $\Omega = P$. Let the buyer's common prior equal to the probability distribution of the prospect, i.e., $\theta_i = p_i$. And let the true underlying distribution $\mu$ satisfy $\frac{\mu_i}{\theta_i} \propto \pi_i$, i.e., $\frac{\mu_i}{\theta_i} = \pi_i \cdot M$ where $M$ is a constant so that $\sum_i \theta_i \pi_i \cdot M = 1$. Finally let the cost of uncertainty be the expected value of the prospect, i.e., $C(\theta) = \E_\theta[v] = \sum_{i=1}^n \theta_i v_i$.\footnote{This is not really a valid cost of uncertainty function, as $C(e_i) \neq 0$ for $e_i = (0,\dots,0, 1, 0, \dots, 0)$. But our algorithm still works when the cost of uncertainty is a linear function. \sherry{May need to check this if the algorithm is updated.}} Then it is easy to verify that~\eqref{optimal_info_dis} is equivalent to the optimal advertising problem~\eqref{prog:opt1} with a constant factor difference in the objective function,
\begin{align*}
&\sum_s \left(\sum_i p_i \sigma(i, s) \cdot \frac{\sum_i p_i \sigma(i, s) \pi_i}{\sum_i p_i \sigma(i, s)}\right)  \frac{\sum_i p_i \sigma(i, s)v_i}{\sum_i p_i \sigma(i, s)} \\
= & \sum_s  \left(\sum_i \theta_i \sigma(i, s) \pi_i\right) \frac{\sum_i \theta_i \sigma(i, s)v_i}{\sum_i \theta_i \sigma(i, s)} \\
= & \sum_s  \left(\sum_i \theta_i \sigma(i, s) \cdot \frac{\mu_i}{\theta_i} /M\right)  C(\eta^s) \\
= & \frac{1}{M} \sum_s  \left(\sum_i \mu_i \sigma(i, s) \right)  C(\eta^s).
\end{align*}

\end{comment}
